Phase-space methods for representing, manipulating, and correcting Gottesman-Kitaev-Preskill qubits

The Gottesman-Kitaev-Preskill (GKP) encoding of a qubit into a bosonic mode is a promising bosonic code for quantum computation due to its tolerance for noise and all-Gaussian gate set. We present a toolkit for phase-space description and manipulation of GKP encodings that includes Wigner functions for ideal and approximate GKP states, for various types of mixed GKP states, and for GKP-encoded operators. One advantage of a phase-space approach is that Gaussian unitaries, required for computation with GKP codes, correspond to simple transformations on the arguments of Wigner functions. We use this fact and our toolkit to describe GKP error correction, including magic-state preparation, entirely in phase space using operations on Wigner functions. While our focus here is on the square-lattice GKP code, we provide a general framework for GKP codes defined on any lattice.

==> WEC updated for arxiv (Comments stripped)/Menicucci_preamble.tex <==
%
%
%
%
%


\allowdisplaybreaks[4]

\graphicspath{{./figures/}}

\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\TR}{TR}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\spur}{sp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Herm}{Herm}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\Prob}{Prob}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\sinc}{sinc}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}

\newcommand{\diffd}{\mathrm{d}}

%
%
%

%
\makeatletter

%
%

%
\newcommand{\ringplus}{\mathbin{\text{\@ringplus}}}

\newcommand{\@ringplus}{%
  \ooalign{\hidewidth\raise1.3ex\hbox{\tiny$\circ$}\hidewidth\cr$\m@th+$\cr}%
}

\newcommand{\ringminus}{\mathbin{\text{\@ringminus}}}

\newcommand{\@ringminus}{%
  \ooalign{\hidewidth\raise0.9ex\hbox{\tiny$\circ$}\hidewidth\cr$\m@th-$\cr}%
}
\makeatother
%

\newcommand{\rplus}{{\ringplus}}
\newcommand{\rminus}{{\ringminus}}

\newcommand{\nasc}{\epsilon}
\newcommand{\dnasc}{\delta_\nasc}
\newcommand{\tdnasc}{\tilde \delta_\nasc}

\newcommand{\qnasc}{q_\nasc}
\newcommand{\pnasc}{p_\nasc}


\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\const}[0]{\text{(const.)}}
\newcommand{\cc}[0]{\text{c.c.}}
\newcommand{\bvec}[1]{\bm{#1}}

\newcommand{\tp}[0]{\mathrm{T}}
\newcommand{\herm}[0]{\mathrm{H}}
\newcommand{\psinv}[0]{+}

\newcommand{\group}[1]{\mathrm{{#1}}}
\newcommand{\algebra}[1]{\mathfrak{{#1}}}
\newcommand{\logical}[0]{L}

\newcommand{\mathlatt}[1]{{\mathsf{#1}}}
\newcommand{\mathreclatt}[1]{\tilde{\mathsf{#1}}}
\newcommand{\dirlatt}{{\mathlatt L}}
\newcommand{\reclatt}{{\tilde \dirlatt}}
\newcommand{\vlatt}{{\mathlatt V}}
\newcommand{\flatt}{{\mathlatt F}}
\newcommand{\slatt}{{\mathlatt S}}


\newcommand{\weyl}{V}


%
%
%

\DeclareFontFamily{U}{wncy}{}
\DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
\DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
\DeclareMathSymbol{\Sh}{\mathord}{mcy}{"58}



%
%
%

%

%
\newcommand{\negspace}{\!}
%

%
\newcommand{\lsub}[2]{{\protect\vphantom{#1}}_{#2} \negspace {#1}}
\newcommand{\rsub}[2]{{#1} \negspace {\protect\vphantom{#1}}_{#2}}
\newcommand{\lrsub}[3]{{\protect\vphantom{#1}}_{#2} \negspace {#1} \negspace {\protect\vphantom{#1}}_{#3}}

%
\newcommand{\ketsub}[2]{\rsub {\ket{#1}} {#2}}
\newcommand{\brasub}[2]{\lsub {\bra{#1}} {#2}}

%
\newcommand{\pbra}[1]{\brasub{#1} p}
\newcommand{\qbra}[1]{\brasub{#1} q}
\newcommand{\pket}[1]{\ketsub{#1} p}
\newcommand{\qket}[1]{\ketsub{#1} q}

%
\newcommand{\inprod}[2]{\left\langle {#1} | {#2} \right\rangle}
%
\newcommand{\mathinprod}[2]{\avg{{#1},{#2}}}

%
\newcommand{\inprodsubsub}[4]{\lrsub {\inprod{#1}{#2}} {#3} {#4}}

%
\newcommand{\pqinprod}[2]{\inprodsubsub{#1}{#2} p q}
\newcommand{\qpinprod}[2]{\inprodsubsub{#1}{#2} q p}
\newcommand{\pinprod}[2]{\inprodsubsub{#1}{#2} p p}
\newcommand{\qinprod}[2]{\inprodsubsub{#1}{#2} q q}

%
\newcommand{\outprod}[2]{\ket {#1}\!\bra {#2}}

%
\newcommand{\outprodsubsub}[4]{\ketsub {#1}{#3} \brasub{#2}{#4}}

%
\newcommand{\pqoutprod}[2]{\outprodsubsub{#1}{#2}p q}
\newcommand{\qpoutprod}[2]{\outprodsubsub{#1}{#2}q p}
\newcommand{\qoutprod}[2]{\outprodsubsub{#1}{#2}q q}
\newcommand{\poutprod}[2]{\outprodsubsub{#1}{#2}p p}


%
%
%


%
\newcommand{\pnascbra}[1]{\brasub{#1} \pnasc}
\newcommand{\qnascbra}[1]{\brasub{#1} \qnasc}
\newcommand{\pnascket}[1]{\ketsub{#1} \pnasc}
\newcommand{\qnascket}[1]{\ketsub{#1} \qnasc}

%
\newcommand{\pqnascinprod}[2]{\inprodsubsub{#1}{#2} \pnasc \qnasc}
\newcommand{\qpnascinprod}[2]{\inprodsubsub{#1}{#2} \qnasc \pnasc}
\newcommand{\pnascinprod}[2]{\inprodsubsub{#1}{#2} \pnasc \pnasc}
\newcommand{\qnascinprod}[2]{\inprodsubsub{#1}{#2} \qnasc \qnasc}

%
\newcommand{\pqnascoutprod}[2]{\outprodsubsub{#1}{#2}\pnasc \qnasc}
\newcommand{\qpnascoutprod}[2]{\outprodsubsub{#1}{#2}\qnasc \pnasc}
\newcommand{\qnascoutprod}[2]{\outprodsubsub{#1}{#2}\qnasc \qnasc}
\newcommand{\pnascoutprod}[2]{\outprodsubsub{#1}{#2}\pnasc \pnasc}



%
%
%



\newcommand{\opbra}[1]{\left( {#1} \right\rvert}
\newcommand{\opket}[1]{\left\lvert {#1} \right)}
\newcommand{\opinprod}[2]{\left( {#1} \middle\vert {#2} \right)}
\newcommand{\opoutprod}[2]{\opket {#1} \opbra {#2}}



\newcommand{\avg}[1]{\left\langle {#1} \right\rangle}
\newcommand{\avgg}[1]{\langle {#1} \rangle}
\newcommand{\abs}[1]{\left\lvert{#1}\right\rvert}
\newcommand{\abss}[1]{\lvert{#1}\rvert}
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}
\newcommand{\normm}[1]{\lVert{#1}\rVert}



\newcommand{\fpart}[1]{\left\{{#1}\right\}}
\newcommand{\fpartt}[1]{\{{#1}\}}

%
%

\newcommand{\ipart}[1]{\left\lfloor{#1}\right\rceil}
\newcommand{\ipartt}[1]{\lfloor{#1}\rceil}


\DeclareMathOperator{\pv}{p.v.}


\newcommand{\reals}[0]{\mathbb{R}}
\newcommand{\complex}[0]{\mathbb{C}}
\newcommand{\wholenums}[0]{\mathbb{N}_0}
\newcommand{\integers}[0]{\mathbb{Z}}
\newcommand{\rationals}[0]{\mathbb{Q}}
\newcommand{\projective}{\mathbb{P}}


\newcommand{\op}[1]{\hat{#1}}
\newcommand{\ope}[1]{\hat{#1}}
%
\newcommand{\opvec}[1]{\op{\vec{#1}}}
\newcommand{\opmat}[1]{\op{\mat{#1}}}
%
\newcommand{\id}[0]{I}
\newcommand{\supop}[1]{\mathcal{#1}}

%

%

%
%
\newcommand{\mat}[1]{\bm{\mathrm{#1}}}
\newcommand{\barmat}[1]{\bar{\mat{#1}}}
\newcommand{\tildemat}[1]{\tilde{\mat{#1}}}
%
\newcommand{\barvec}[1]{\bar{\vec{#1}}}
\newcommand{\tildevec}[1]{\tilde{\vec{#1}}}

\renewcommand{\vec}[1]{\bm{\mathrm{#1}}}
%

\newcommand{\controlled}[1]{\op{\mathrm{C}}_{#1}}
\newcommand{\CZ}[0]{\controlled Z}
\newcommand{\CX}[0]{\controlled X}
\newcommand{\CZct}[0]{\controlled Z^\rightarrow}
\newcommand{\CXct}[0]{\controlled X^\rightarrow}
\newcommand{\CZtc}[0]{\controlled Z^\leftarrow}
\newcommand{\CXtc}[0]{\controlled X^\leftarrow}

\newcommand{\opCZ}[0]{\op{\mathrm{C}}_{Z}}

\newcommand{\cH}[0]{\mathcal{H}}






%
%
%
\newcommand{\grn}{\color{green!60!black}}
\newcommand{\red}{\color{red!90!black}}
\newcommand{\blu}{\color{blue!70!cyan}}
\newcommand{\blk}{\color{black}}
\newcommand{\gra}{\color{gray!50!white}}
\newcommand{\prp}{\color{purple!70!black}}
\newcommand{\org}{\color{orange!80!black}}
\newcommand{\pnk}{\color{pink}}

%
%
%

\endinput

